Robust Parameter Inversion using Adaptive Reduced Order Models

Nonlinear parametric inverse problems appear in many applications and are typically very expensive to solve, especially if they involve many measurements. These problems pose huge computational challenges as evaluating the objective function or misfit requires the solution of a large number of parameterized partial differential equations, typically one per source term. Newton-type algorithms, which may be required for fast convergence, typically require the additional solution of a large number of adjoint problems. The use of parametric model reduction may substantially alleviate this problem. In [de Sturler, E., Gugercin, S., Kilmer, M. E., Chaturantabut, S., Beattie, C., and O'Connell, M. (2015). Nonlinear Parametric Inversion Using Interpolatory Model Reduction. SIAM Journal on Scientific Computing, 37(3)], interpolatory model reduction was successfully used to drastically speed up inversion for Diffuse Optical Tomography (DOT). However, when using model reduction in high dimensional parameter spaces, obtaining error bounds in parameter space is typically intractable. In this paper, we propose to use stochastic estimates to remedy this problem. At the cost of one (randomized) full-scale linear solve per optimization step we obtain a robust algorithm. Moreover, since we can now update the model when needed, this robustness allows us to further reduce the order of the reduced order model and hence the cost of computing and using it, further decreasing the cost of inversion. We also propose a method to update the model reduction basis that reduces the number of large linear solves required by 46%-98% compared with the fixed reduced-order model. We demonstrate that this leads to a highly efficient and robust inversion method.

==> assets/amoeba_results_5_permille.tex <==
\begin{table}[ht]%
\begin{tabular}{|l|c|r@{\hspace{.25em}}c@{\hspace{.25em}}r@{\hspace{.5em}}r|}%
\hline%
Experiment Setup&Large Solves&\multicolumn{4}{c|}{Smaller Solves}\\%
&{[}Amortized{]}&&&&\\%
\hline%
\multirow{1}{*}{Full Order Model}&1856 {[}1792{]}&&&&\\%
\hline%
\multirow{3}{*}{ROM - 1 Step - Interpolatory Updates at $\V{x}_\mathrm{c}$}&212 {[}148{]}&64&$\times$&64:&256\\%
&&88&$\times$&88:&352\\%
&&106&$\times$&106:&224\\%
\hline%
\multirow{3}{*}{ROM - 1 Step - Interpolatory Updates at $\V{{x}}_\mathrm{p}$}&219 {[}155{]}&64&$\times$&64:&256\\%
&&88&$\times$&88:&576\\%
&&104&$\times$&104:&288\\%
\hline%
\multirow{3}{*}{ROM - 1 Step - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&102 {[}38{]}&64&$\times$&64:&256\\%
&&70&$\times$&70:&416\\%
&&76&$\times$&76:&448\\%
\hline%
\multirow{3}{*}{ROM - 1 Step - Residual-Driven Updates at $\V{{x}}_\mathrm{p}$}&95 {[}31{]}&64&$\times$&64:&256\\%
&&70&$\times$&70:&416\\%
&&76&$\times$&76:&160\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Interpolatory Updates at $\V{x}_\mathrm{c}$}&341 {[}277{]}&80&$\times$&80:&256\\%
&&102&$\times$&102:&672\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Interpolatory Updates at $\V{{x}}_\mathrm{p}$}&338 {[}274{]}&80&$\times$&80:&256\\%
&&102&$\times$&102:&512\\%
\hline%
\multirow{1}{*}{ROM - 3 Step - No Updates}&273 {[}209{]}&80&$\times$&80:&768\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&280 {[}216{]}&80&$\times$&80:&256\\%
&&84&$\times$&84:&608\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Residual-Driven Updates at $\V{{x}}_\mathrm{p}$}&277 {[}213{]}&80&$\times$&80:&256\\%
&&84&$\times$&84:&480\\%
\hline%
\end{tabular}%
\caption{Number of Linear Solves for the 2D Problem}%
\label{table:2D_results}%
\end{table}

==> assets/torus_results_5_permille.tex <==
\begin{table}[ht]%
\begin{tabular}{|l|c|r@{\hspace{.25em}}c@{\hspace{.25em}}r@{\hspace{.5em}}r|}%
\hline%
Experiment Setup&Large Solves&\multicolumn{4}{c|}{Smaller Solves}\\%
&{[}Amortized{]}&&&&\\%
\hline%
\multirow{1}{*}{Full Order Model}&28830 {[}26908{]}&&&&\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Interpolatory Updates}&3863 {[}1941{]}&1922&$\times$&1922:&20181\\%
&&2092&$\times$&2092:&8649\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Residual-Driven Updates}&1967 {[}45{]}&1922&$\times$&1922:&20181\\%
&&1948&$\times$&1948:&8649\\%
\hline%
\multirow{1}{*}{ROM - 3 Step - Interpolatory Updates}&8654 {[}6732{]}&1950&$\times$&1950:&8649\\%
\hline%
\multirow{1}{*}{ROM - 3 Step - No Updates}&8654 {[}6732{]}&1950&$\times$&1950:&8649\\%
\hline%
\multirow{1}{*}{ROM - 3 Step - Residual-Driven Updates}&8654 {[}6732{]}&1950&$\times$&1950:&8649\\%
\hline%
\end{tabular}%
\caption{Number of Linear Solves for the 3D Problem}%
\label{table:3D_results}%
\end{table}

==> post/2D_1_permille_results.tex <==
\begin{table}[ht]%
\begin{tabular}{|l|c|c|c|c|c|}%
\hline%
\multirow{2}{*}{Experiment Setup}&Median Solves&\multicolumn{4}{c|}{Percentiles}\\%
\cline{3%
-%
6}%
&{[}Amortized{]}&Min&25&75&Max\\%
\hline%
\multirow{2}{*}{Full Order Model}&992&704&896&1120&2240\\%
&{[}928{]}&{[}640{]}&{[}832{]}&{[}1056{]}&{[}2176{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 3 Point - Interpolatory Updates at $\V{x}_\mathrm{c}$}&279&207&274&283&373\\%
&{[}215{]}&{[}143{]}&{[}210{]}&{[}219{]}&{[}309{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 3 Point - Interpolatory Updates at $\V{x}_\mathrm{p}$}&279&207&274&283&360\\%
&{[}215{]}&{[}143{]}&{[}210{]}&{[}219{]}&{[}296{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 3 Point - No Updates}&192&192&192&192&192\\%
&{[}128{]}&{[}128{]}&{[}128{]}&{[}128{]}&{[}128{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 3 Point - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&219&207&215&223&245\\%
&{[}155{]}&{[}143{]}&{[}151{]}&{[}159{]}&{[}181{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 3 Point - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&218&207&215&223&244\\%
&{[}154{]}&{[}143{]}&{[}151{]}&{[}159{]}&{[}180{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 1 Point - Interpolatory Updates at $\V{x}_\mathrm{c}$}&302&213&229&308&444\\%
&{[}238{]}&{[}149{]}&{[}165{]}&{[}244{]}&{[}380{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 1 Point - Interpolatory Updates at $\V{x}_\mathrm{p}$}&240&214&230&302&311\\%
&{[}176{]}&{[}150{]}&{[}166{]}&{[}238{]}&{[}247{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 1 Point - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&138&107&133&140&155\\%
&{[}74{]}&{[}43{]}&{[}69{]}&{[}76{]}&{[}91{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 1 Point - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&132&101&125&135&145\\%
&{[}68{]}&{[}37{]}&{[}61{]}&{[}71{]}&{[}81{]}\\%
\hline%
\end{tabular}%
\caption{Number of Large Linear Solves for the 2D Problem}%
\label{table:2D_results}%
\end{table}

==> post/2D_5_permille_results.tex <==
\begin{table}[ht]%
\begin{tabular}{|l|c|c|c|c|c|}%
\hline%
\multirow{2}{*}{Experiment Setup}&Median Solves&\multicolumn{4}{c|}{Percentiles}\\%
\cline{3%
-%
6}%
&{[}Amortized{]}&Min&25&75&Max\\%
\hline%
\multirow{2}{*}{Full Order Model}&736&416&672&800&1088\\%
&{[}672{]}&{[}352{]}&{[}608{]}&{[}736{]}&{[}1024{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Interpolatory Updates at $\V{x}_\mathrm{c}$}&205&199&204&207&280\\%
&{[}141{]}&{[}135{]}&{[}140{]}&{[}143{]}&{[}216{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Interpolatory Updates at $\V{x}_\mathrm{p}$}&205&199&204&207&280\\%
&{[}141{]}&{[}135{]}&{[}140{]}&{[}143{]}&{[}216{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - No Updates}&192&192&192&192&192\\%
&{[}128{]}&{[}128{]}&{[}128{]}&{[}128{]}&{[}128{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&205&199&204&207&220\\%
&{[}141{]}&{[}135{]}&{[}140{]}&{[}143{]}&{[}156{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&205&201&204&207&220\\%
&{[}141{]}&{[}137{]}&{[}140{]}&{[}143{]}&{[}156{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Interpolatory Updates at $\V{x}_\mathrm{c}$}&215&144&212&220&414\\%
&{[}151{]}&{[}80{]}&{[}148{]}&{[}156{]}&{[}350{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Interpolatory Updates at $\V{x}_\mathrm{p}$}&215&143&213&217&230\\%
&{[}151{]}&{[}79{]}&{[}149{]}&{[}153{]}&{[}166{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&101&89&99&106&114\\%
&{[}37{]}&{[}25{]}&{[}35{]}&{[}42{]}&{[}50{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&99&85&96&101&119\\%
&{[}35{]}&{[}21{]}&{[}32{]}&{[}37{]}&{[}55{]}\\%
\hline%
\end{tabular}%
\caption{Number of Large Linear Solves for the 2D Problem}%
\label{table:2D_results}%
\end{table}

==> post/3D_1_permille_results.tex <==
\begin{table}[ht]%
\begin{tabular}{|l|c|c|c|c|c|}%
\hline%
\multirow{2}{*}{Experiment Setup}&Median Solves&\multicolumn{4}{c|}{Percentiles}\\%
\cline{3%
-%
6}%
&{[}Amortized{]}&Min&25&75&Max\\%
\hline%
\multirow{2}{*}{Full Order Model}&23064&16337&22103&24025&26908\\%
&{[}21142{]}&{[}14415{]}&{[}20181{]}&{[}22103{]}&{[}24986{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 3 Point - Interpolatory Updates at $\V{x}_\mathrm{p}$}&5776&5774&5775&5776&7704\\%
&{[}3854{]}&{[}3852{]}&{[}3853{]}&{[}3854{]}&{[}5782{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 3 Point - No Updates}&5766&5766&5766&5766&5766\\%
&{[}3844{]}&{[}3844{]}&{[}3844{]}&{[}3844{]}&{[}3844{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 3 Point - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&5776&5774&5775&5777&5797\\%
&{[}3854{]}&{[}3852{]}&{[}3853{]}&{[}3855{]}&{[}3875{]}\\%
\hline%
\multirow{2}{4.6cm}{ROM - 1 Point - Interpolatory Updates at $\V{x}_\mathrm{p}$}&3871&3858&3867&3881&5798\\%
&{[}1949{]}&{[}1936{]}&{[}1945{]}&{[}1959{]}&{[}3876{]}\\%
\hline%
\multirow{2}{4.75cm}{ROM - 1 Point - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&1985&1953&1965&1993&2006\\%
&{[}63{]}&{[}31{]}&{[}43{]}&{[}71{]}&{[}84{]}\\%
\hline%
\end{tabular}%
\caption{Number of Large Linear Solves for the 3D Problem}%
\label{table:3D_results}%
\end{table}

==> post/3D_5_permille_results.tex <==
\begin{table}[ht]%
\begin{tabular}{|l|c|c|c|c|c|}%
\hline%
\multirow{2}{*}{Experiment Setup}&Median Solves&\multicolumn{4}{c|}{Percentiles}\\%
\cline{3%
-%
6}%
&{[}Amortized{]}&Min&25&75&Max\\%
\hline%
\multirow{2}{*}{Full Order Model}&15376&15376&15376&15376&15376\\%
&{[}13454{]}&{[}13454{]}&{[}13454{]}&{[}13454{]}&{[}13454{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Interpolatory Updates at $\V{x}_\mathrm{c}$}&5771&5771&5771&5771&5771\\%
&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Interpolatory Updates at $\V{x}_\mathrm{p}$}&5771&5771&5771&5771&5771\\%
&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - No Updates}&5766&5766&5766&5766&5766\\%
&{[}3844{]}&{[}3844{]}&{[}3844{]}&{[}3844{]}&{[}3844{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&5771&5771&5771&5771&5771\\%
&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}\\%
\hline%
\multirow{2}{*}{ROM - 3 Step - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&5771&5771&5771&5771&5771\\%
&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}&{[}3849{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Interpolatory Updates at $\V{x}_\mathrm{c}$}&3862&3862&3862&3862&3862\\%
&{[}1940{]}&{[}1940{]}&{[}1940{]}&{[}1940{]}&{[}1940{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Interpolatory Updates at $\V{x}_\mathrm{p}$}&3863&3863&3863&3863&3863\\%
&{[}1941{]}&{[}1941{]}&{[}1941{]}&{[}1941{]}&{[}1941{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Residual-Driven Updates at $\V{x}_\mathrm{c}$}&1961&1961&1961&1961&1961\\%
&{[}39{]}&{[}39{]}&{[}39{]}&{[}39{]}&{[}39{]}\\%
\hline%
\multirow{2}{*}{ROM - 1 Step - Residual-Driven Updates at $\V{x}_\mathrm{p}$}&1972&1972&1972&1972&1972\\%
&{[}50{]}&{[}50{]}&{[}50{]}&{[}50{]}&{[}50{]}\\%
\hline%
\end{tabular}%
\caption{Number of Large Linear Solves for the 3D Problem}%
\label{table:3D_results}%
\end{table}
